Consistent Estimators for Learning to Defer to an Expert

Learning algorithms are often used in conjunction with expert decision makers in practical scenarios, however this fact is largely ignored when designing these algorithms. In this paper we explore how to learn predictors that can either predict or choose to defer the decision to a downstream expert. Given only samples of the expert's decisions, we give a procedure based on learning a classifier and a rejector and analyze it theoretically. Our approach is based on a novel reduction to cost sensitive learning where we give a consistent surrogate loss for cost sensitive learning that generalizes the cross entropy loss. We show the effectiveness of our approach on a variety of experimental tasks.

==> chexpert.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Chest X-Ray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Task.} CheXpert is a large chest radiograph dataset that contains over 224 thousand images of 65,240 patients automatically labeled for the presence of 14 observations using radiology reports \cite{irvin2019chexpert}. In addition to the automatically labeled training set, \cite{irvin2019chexpert} make publicly accessible a validation set of 200 patients labeled by a consensus of 3 radiologists and hide a further testing set of 500 patients labeled by 8 radiologists. We focus here on the detection of only the 5 observations that make up the "competition tasks" \cite{irvin2019chexpert}: Atelectasis, Cardiomegaly,  Consolidation, Edema, and Pleural Effusion. This is a multi-task problem, we have 5 separate binary tasks, we will learn to defer on an individual task basis.

\subsubsection{Expert models}
 We conduct experiments with two experts: the first is a toy expert where we can identify the correct deferral behavior and the second set of experts tries to emulate actual radiologist behavior. 

\textbf{1) Toy expert.} We create a simulated expert as follows: if the chest X-ray contains support devices (the presence of support devices is part of the label) then the expert is correct with probability $p$ on all tasks independently and if the X-ray does not contain support devices, then the expert is correct with probability $q$. We vary $q \in \{0.5,0.7\}$ and  $p \in \{0.7,0.8,0.9,1\}$ to obtain different experts, we let $p\geq q$ as one can think that a patient that has support devices might have a previous medical history that the expert is aware of and can use as side-information. 

\textbf{2) Radiologist expert.} The hidden test set of 500 patients was labeled by 8 radiologists: the consensus of 5 of them constituted the ground truth label and the annotation of the remaining 3 were used to benchmark radiologist performance. We obtained the ground truth label and the 3 radiologist annotations that were used to benchmark on the test set without the input images. Using  this test data we learn  models of radiologist behavior to use as our expert.
The test data consists of the following tuples $D =\{y_i,e_{1,i},e_{2,i},e_{3,i}\}_{i=1}^{500}$, where $y_i \in \{0,1\}^{14}$ is the ground truth data, $e_{1,i},e_{2,i},e_{3,i} \in  \{0,1\}^{14}$ are radiologist 1,2 and 3 predictions respectively, the goal is to learn expert models $\hat{e}_1,\hat{e}_2,\hat{e}_3: \{0,1\}^{14} \to \{0,1\}^{14}$ which map a ground truth label to the radiologists predictions. We decompose $\hat{e}_i$ into 14 different components $\hat{e}_i^j:\{0,1\}^{14}  \to \{0,1\}$ (for each of the 14 tasks, $j \in [14]$) and learn each separately.
We evaluate different strategies to learn the expert models: (1) a class conditional noise model (CCN) of the expert based on the task label, (2) a table lookup from the empirical probabilities of $e_i(j)$ ($j$'th component of expert predictions) given the complete label vector $y$, (3) a logistic regression model treating the label vector $y$ as the covariates and $e_i(j)$ as the target (LR) and finally (4) a random forest classifier (RF). \\
\textit{Evaluation of the strategies.} We use 400 patients to train and 100 patients to test the performance of the strategies, and repeat for 50 trials with different random splits to average out the randomness in the models and data. We look in Table \ref{tab:model_rad_behavior} at the area under the ROC curve (AU-ROC) of the expert models at predicting the radiologists decisions for all 3 radiologists and in Table \ref{tab:model_rad_performance} at the average difference between the performance of the expert models in terms of false positive and true positive rates (FPR,TPR) and F1 at predicting the target and the performance of the actual radiologists. The LR, RF and table lookup method perform similarly at the task of predicting the radiologist decisions  outperforming the naive CCN method, the table lookup method achieves an average AU-ROC of 0.69 over the 5 tasks for radiologist 1. Additionally, all methods are able to match the FPR of the actual experts with an approximate margin of $\pm 0.05$ and the TPR by a margin of $\pm 0.1$ on average across the 3 radiologists. We use the table lookup to construct our expert model for it's simplicity. 



\begin{table}[h]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
         &\textbf{Atelectasis} &  \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Edema} & \textbf{Pleural Effusion}  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 1}} \\ \midrule      
        CCN  & 0.629, (0.585, 0.663)& 0.634, (0.601, 0.664)& 0.568, (0.528, 0.603)& 0.645, (0.606, 0.681)& 0.781, (0.748, 0.806) \\
         \hline
         table lookup & 0.654, (0.613, 0.7)& 0.667, (0.643, 0.701)& 0.625, (0.596, 0.662)& 0.715, (0.695, 0.732)& 0.806, (0.775, 0.841) \\ \hline 
         
      LR &0.646, (0.606, 0.692)& 0.638, (0.606, 0.675)& 0.624, (0.569, 0.669)& 0.719, (0.674, 0.757)& 0.791, (0.761, 0.819) \\ \hline
      
        RF & 0.638, (0.598, 0.67)& 0.657, (0.627, 0.677)& 0.637, (0.593, 0.679)& 0.720, (0.688, 0.753)& 0.806, (0.781, 0.831) \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 2}} \\ \midrule      
        CCN  & 0.672, (0.642, 0.708)& 0.622, (0.592, 0.643)& 0.540, (0.489, 0.574)& 0.633, (0.601, 0.658)& 0.656, (0.631, 0.688) \\
         \hline
         table lookup & 0.697, (0.673, 0.726)& 0.680, (0.643, 0.709)& 0.609, (0.571, 0.65)& 0.668, (0.634, 0.7)& 0.726, (0.691, 0.752) \\ \hline 
         
      LR &0.688, (0.65, 0.713)& 0.669, (0.645, 0.694)& 0.597, (0.532, 0.655)& 0.652, (0.613, 0.691)& 0.710, (0.678, 0.748) \\ \hline
      
        RF &0.702, (0.673, 0.73)& 0.684, (0.643, 0.703)& 0.617, (0.573, 0.66)& 0.672, (0.643, 0.698)& 0.724, (0.687, 0.754) \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 3}} \\ \midrule      
        CCN  & 0.681, (0.631, 0.711)& 0.636, (0.594, 0.671)& 0.571, (0.508, 0.62)& 0.662, (0.631, 0.69)& 0.726, (0.708, 0.735) \\
         \hline
         table lookup & 0.682, (0.636, 0.711)& 0.658, (0.603, 0.707)& 0.594, (0.539, 0.645)& 0.754, (0.722, 0.775)& 0.792, (0.768, 0.822) \\ \hline 
         
      LR &0.700, (0.662, 0.729)& 0.657, (0.614, 0.699)& 0.618, (0.528, 0.689)& 0.758, (0.73, 0.781)& 0.785, (0.76, 0.807) \\ \hline
      
        RF & 0.686, (0.657, 0.714)& 0.679, (0.653, 0.702)& 0.606, (0.539, 0.672)& 0.774, (0.758, 0.789)& 0.795, (0.768, 0.816)
     \\  \bottomrule
    \end{tabular}}
    
    \caption{Average AU-ROC and (25,75) quantiles AU-ROC over the trials of the models at predicting the radiologists predictions for each of the three.}
    \label{tab:model_rad_behavior}
\end{table}








\begin{table}[h]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
         &\textbf{Atelectasis} &  \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Edema} & \textbf{Pleural Effusion}  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 1}} \\ \midrule      
        CCN  & (0.029,0.109), 0.100 & (0.040,0.138), 0.120  & (0.035,0.232), 0.104  & (0.053,0.068), 0.056  & (0.032,0.105), 0.085 \\
         \hline
         table lookup & (0.030,0.124), 0.105 & (0.035,0.113), 0.104  & (0.028,0.252), 0.108  & (0.047,0.073), 0.052  & (0.027,0.110), 0.079 \\ \hline 
         
      LR &(0.031,0.111), 0.097 & (0.034,0.156), 0.122  & (0.035,0.268), 0.135  & (0.043,0.088), 0.056  & (0.022,0.122), 0.086  \\ \hline
      
        RF & (0.034,0.127), 0.120 & (0.032,0.150), 0.118  & (0.034,0.249), 0.115  & (0.043,0.075), 0.048  & (0.022,0.112), 0.079  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 2}} \\ \midrule      
        CCN  & (0.062,0.076), 0.062 & (0.046,0.106), 0.082  & (0.027,0.286), 0.164  & (0.054,0.105), 0.080  & (0.048,0.096), 0.069   \\
         \hline
         table lookup & (0.056,0.059), 0.050 & (0.051,0.106), 0.085  & (0.030,0.222), 0.135  & (0.051,0.095), 0.066  & (0.052,0.093), 0.077  \\ \hline 
         
      LR &(0.050,0.071), 0.044 & (0.056,0.102), 0.083  & (0.033,0.232), 0.147  & (0.051,0.108), 0.082  & (0.054,0.094), 0.070 \\ \hline
      
        RF &(0.060,0.081), 0.058 & (0.045,0.110), 0.070  & (0.027,0.240), 0.156  & (0.047,0.092), 0.062  & (0.044,0.093), 0.069  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 3}} \\ \midrule      
                CCN  &(0.037,0.112), 0.079 & (0.035,0.165), 0.130  & (0.021,0.262), 0.214  & (0.069,0.054), 0.046  & (0.042,0.070), 0.066 \\
         \hline
         table lookup & (0.049,0.101), 0.080 & (0.033,0.131), 0.117  & (0.020,0.252), 0.204  & (0.056,0.063), 0.050  & (0.036,0.085), 0.059 \\ \hline 
         
      LR &(0.044,0.096), 0.079 & (0.038,0.165), 0.130  & (0.023,0.247), 0.194  & (0.062,0.060), 0.046  & (0.038,0.092), 0.064  \\ \hline
      
        RF &(0.044,0.105), 0.077 & (0.030,0.154), 0.117  & (0.040,0.240), 0.226  & (0.054,0.054), 0.039  & (0.033,0.083), 0.052 
      \\  \bottomrule
    \end{tabular}}
    
    \caption{Average absolute difference between the (FPR,TPR) of the expert model at predicting the target and that of the actual radiologists along with the absolute difference of F1 score. }
    \label{tab:model_rad_performance}
\end{table}

\subsubsection{Experimental details}

\textbf{Data.} We use the downsampled resolution version of CheXpert \cite{irvin2019chexpert} and split the training data set with an 80-10-10 split on a patient basis for training, validation and testing respectively, no patients are shared among the splits. Images are normalized and resized to be compatible with pre-trained ImageNet models, we use data augmentation in the form of random resized crops, horizontal flips and random rotations of up to $15\degree$  while training. For the radiologist experts use the expert model "table lookup" learned to label this data with expert predictions for each of the 3 radiologists. Note that
a small subset of the training data has an uncertainty label "U" instead of a binary label that implies that the automatic annotator is uncertain, we ignore these points on a task basis while training and testing, however to obtain the expert label for these points (for tasks that don't have an uncertainty label) we replace "U" by a "1" label. 



\textbf{Baselines.} We implement two baselines: a threshold confidence baseline that learns a threshold to maximize system AU-ROC on just the confidence of the classifier model to defer (ModelConfidence), this is the post-hoc thresholding method in \cite{madras2018predict}, and the Confidence baseline \cite{raghu2019algorithmic}. We use temperature scaling \cite{guo2017calibration} to ensure calibration of all baselines on the validation set. 


\textbf{Model.} Following \cite{irvin2019chexpert}, we use the DenseNet121 architecture for our model with pre-trained weights on ImageNet, the loss for the baseline models is the average of the binary cross entropy for each of the tasks. We train the baseline models using Adam for 4 epochs. For our approach we train for 3 epochs using the cross entropy loss  and then train for one epoch using $L_{CE}^\alpha$ with $\alpha$ chosen to maximize the area under the receiver operating characteristic curve (AU-ROC) of the combined system on the validation set for each of the 5 tasks (each task is treated separately). We also observe similar results if we train for the first three epochs with $L_{CE}^1$ and then train for one epoch with a validated choice of $\alpha$.

\textbf{Experimental setup.} In a clinical setting there might be a cost associated to querying a radiologist, this then imposes a constraint on how often we can query the radiologist i.e. our model's coverage (fraction of examples where algorithm predicts). We constrain our method and the baselines to achieve $c\%$ coverage for $c \in [100]$ to simulate the spectrum between complete automation and none.\\
We achieve this for our method by first sorting the test set based on  $g_{\bot}(x) - \max(g_0(x),g_1(x)):=q(x)$ across all patients $x$ in the test set, then to achieve coverage $c$, we define $\tau = q(x_c)$ where $q(x_c)$ is the $c$'th percentile of the outputs $q(x)$, then we let $r(x) =1 \iff q(x) \geq \tau$. The definition of $\tau$ ensures that we obtain exactly $c\%$ coverage.

For ModelConfidence we achieve this by letting $q(x) = 1- \max(g_0(x),g_1(x))$ ($g$ is the result of a separate trained model than the one for our method), this is the natural classifier's probability of error from the softmax output, and for the Confidence we let $q(x)$ be the difference between the radiologists confidence and  the classifier's confidence.

\subsubsection{Results and Analysis}
\textbf{Results for toy expert.} In Figure \ref{fig:auc_vs_cov_toy} we plot the overall system (expert and algorithm combined) AU-ROC for each desired coverage for the methods and in Figure \ref{fig:ap_vs_cov_toy} we plot the overall system area under the precision-recall curve (AU-PR) versus the coverage; this is for the expert with $q=0.7$ and $p=1$. We can see that the curve for our method dominates the baselines over the entire coverage range for both AU-ROC and AU-PR, moreover the curves are concave and we can achieve higher performance by combining expert and algorithm than using both separately. Our method is able to achieve a higher maximum AU-ROC and AU-PR than both baselines: the difference between the maximum attainable AU-ROC of our method and Confidence is 0.043, 0.029, 0.016, 0.022 and 0.025 respectively for each of the five tasks.
There is a clear hierarchy between the 3 compared methods: our method dominates Confidence and Confidence in turn dominates ModelConfidence, in fact ModelConfidence is a special case of the Confidence baseline, since the expert does not have uniform performance over the domain there are clear gains in modeling the expert. 

This hierarchy continues to hold as we change the expert behavior as we vary the probabilities $p$ and $q$, in Table \ref{table:toy_expert} we show for each of the 5 tasks the difference between the average AU-ROC across all coverages (average value of the curves shown in Figure \ref{fig:auc_vs_cov_toy}) for our method and the Confidence baseline for different expert probabilities and the difference between the maximum achievable AU-ROC. A positive average difference serves to show the degree of dominance of our method over the Confidence baseline, note that the difference alone cannot imply dominance of the curves however dominance is still observed. Our method improves on the baselines as the difference between $q$ and $p$ increases, this difference encodes the non-uniformity of the expert behavior over the domain.


\begin{figure}[h]
\centering
\begin{subfigure}{.9\textwidth}
\centering

      \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/auc_vs_cov_toyexpert7-1.pdf}
      \caption{AU-ROC vs coverage for expert $q=0.7,p=1$, maximum AU-ROC is noted.}
      \label{fig:auc_vs_cov_toy}
\end{subfigure}

\begin{subfigure}{.9\textwidth}
\centering
  \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/ap_vs_cov_toyexpert7-1.pdf}
\caption{AU-PR vs coverage for expert $q=0.7,p=1$, maximum AU-PR is noted.}
      \label{fig:ap_vs_cov_toy}
\end{subfigure}

\caption{Plot of AU-ROC of the ROC curve (a) for each level of coverage (0 coverage means only the expert predicting and 1 coverage is only the classifier predicting) and of the area under the precision-recall curve (AU-PR) (b) for each of the 5 tasks comparing our method with the baselines on the training derived test set for the toy expert with $q=0.7,p=1$. We report the maximum AU-ROC and AU-PR achieved on each task, error bars are standard deviations derived from 10 runs (averaging over the expert's randomness).}
\label{fig:plots_auc_ap_toyexpert}
\end{figure}




\begin{table}
\caption{Average difference in AU-ROC across all coverage and difference between maximum achievable AU-ROC between our method and the Confidence baseline for each of the 5 tasks and different toy expert probabilities $p$ and $q$; each entry is (average difference $\pm$ standard deviation; difference of maximums). The difference between our method and the ModelConfidence is roughly twice the values noted in table \ref{table:toy_expert}, only at Expert $(0.7,0.7)$ does Confidence and ModelConfidence achieve the same performance since the expert has uniform error over the domain.}
\label{table:toy_expert}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
Expert $(p,q)$ &  \textbf{Cardiomegaly} & \textbf{Edema} & \textbf{Consolidation}  &   \textbf{Atelectasis}  & \textbf{Pleural Effusion}  \\
\midrule
(0.5,0.7) &0.032$\pm$0.024; 0.002  &0.015$\pm$0.012; 0.007    &  0.015$\pm$0.008; 0.007    & 0.017$\pm$0.009; 0.007     & 0.007$\pm$0.003 ;0.007   \\ \hline
(0.5,0.9) & 0.032$\pm$0.017; 0.014 &  0.026$\pm$0.016; 0.024 & 0.010$\pm$0.005; 0.015    &   0.016$\pm$0.008; 0.026   & 0.012$\pm$0.010; 0.004  \\ \hline
(0.5,1)  & 0.022$\pm$0.012; 0.029 & 0.013$\pm$0.009; 0.019  & 0.007$\pm$0.008; 0.012    & 0.013$\pm$0.006; 0.020     & 0.010$\pm$0.008; 0.012   \\ \hline
(0.7,0.7) & 0.024$\pm$0.018; 0.005  & 0.011$\pm$0.009; 0.010  &  0.011$\pm$0.010; 0.009   &  0.006$\pm$0.006; 0.008    &  0.001$\pm$0.001; 0.003  \\ \hline 
(0.7,0.9) & 0.032$\pm$0.020; 0.024   & 0.010$\pm$0.007; 0.010  & 0.007$\pm$0.007; 0.017    &  0.014$\pm$0.008; 0.017    &0.010$\pm$0.006; 0.006   \\ \hline 
(0.7,1) &0.027$\pm$0.014; 0.042  &  0.016$\pm$0.010; 0.027 &  0.007$\pm$0.007; 0.019   &  0.013$\pm$0.007; 0.022    &  0.014$\pm$0.010; 0.027  \\ \hline 
(0.8,1) &  0.017$\pm$0.009; 0.023   & 0.011$\pm$0.008; 0.012   & 0.001$\pm$0.004; 0.007    & 0.012$\pm$0.006; 0.009     & 0.010$\pm$0.006; 0.018 \\ 
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\textbf{Results for radiologist expert.}
In Figure \ref{fig:auc_vs_cov_rad1} we plot the overall system (expert and algorithm combined) AU-ROC for each desired coverage for the methods and in Figure \ref{fig:ap_vs_cov_toy} we plot the overall system area under the precision-recall curve (AU-PR) versus the coverage; this is for for radiologist $\#1$. We can see in figure \ref{fig:auc_vs_cov_rad1} that our method dominates both baselines over the entire coverage range, for example the difference between the average values of AU-ROC across all coverages for our method and Confidence is 0.18 for Cardiomegaly and 0.10 for Edema. The cause of this difference is that both the Confidence and ModelConfidence baselines almost never defer on examples where their prediction is 0, this is due to the class imbalance that causes the classifier to be very confident on the negative class, hence the expert has to predict on the majority of the positive examples. However, the expert has a a low true positive rate on these two tasks that causes the overall performance of the system to drop. With respect to AU-PR in figure \ref{fig:ap_vs_cov_rad1}, our method performs on par with the baselines on Cardiomegaly, Atelectasis and Pleural Effusion. On Edema and Consolidation the average gap between the curves in Figure \ref{fig:ap_vs_cov_rad1} is in the range of $0.01-0.02$. 


\begin{figure}[h]
\centering
\begin{subfigure}{.9\textwidth}
\centering

      \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/auc_vs_cov_rad1.pdf}
      \caption{AU-ROC vs coverage for radiologist $\#1$.}
      \label{fig:auc_vs_cov_rad1}
\end{subfigure}

\begin{subfigure}{.9\textwidth}
\centering
  \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/ap_vs_cov_rad1.pdf}
\caption{AU-PR vs coverage for radiologist $\#1$.}
      \label{fig:ap_vs_cov_rad1}
\end{subfigure}

\caption{Plot of AU-ROC of the ROC curve (a) for each level of coverage (0 coverage means only the expert predicting and 1 coverage is only the classifier predicting) and of the area under the precision-recall curve (AU-PR) (b) for each of the 5 tasks comparing our method with the baselines on the training derived test set for radiologist $\#1$. We report the maximum AU-ROC and AU-PR achieved on each task, error bars are standard deviations derived from 10 runs (averaging over the expert's randomness).}
\label{fig:plots_auc_ap_rad1}
\end{figure}





\subsection{Further Analysis}

\subsection{Sample Complexity}
Training data for chest X-rays is a valuable resource that may not be abundantly available when trying to deploy a machine learning model in a new clinical setting where for example the imaging mechanism may differ. It is important to see the effectiveness of the proposed approaches when training data size is limited, this furthermore helps us understand the comparative sample complexity of our method versus the baselines.


\textbf{Experimental details.} We restrict the training data size for our model and baselines while keeping the same validation and testing data as previously; the validation data is used only for calibration of models and optimizing over choice of $\alpha$. We train using the same procedure as before and report the maximum achievable AU-PR and AU-ROC. The expert we defer to is the synthetic expert described above with $q=0.7$ and $p=1$.


\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={Training data size (as \% of original set)},
    ylabel={mean AU-ROC},
    xmin=0, xmax=100,
    ymin=0.84, ymax=0.93,
    xtick={0,5,10,25,50,75,100},
  ytick={0.85,0.87,0.88,0.89,0.9,0.91,0.92,0.93,0.95},
    legend pos=south west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 \addplot+[
  black, mark options={black, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    5,  0.875,       0.002
    10, 0.876, 0.002
    25, 0.878, 0.002
    50, 0.879, 0.002
    75, 0.88, 0.002
    100, 0.879, 0.002

};
\addlegendentry{ModelConfidence}

 \addplot+[
  blue, mark options={blue, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    5,  0.880,       0.002
    10,  0.883,       0.002
    25,  0.892,       0.002
    50,  0.895,       0.002
    75,  0.9,       0.003
    100,  0.896,       0.003

};
\addlegendentry{Confidence}


 \addplot+[
  red, mark options={red, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    5,  0.889,       0.002
    10,  0.896,       0.002
    25,  0.908,       0.002
    50,  0.914,       0.002
    75,  0.924,       0.002
    100,  0.922,       0.002

};
\addlegendentry{$L_{CE}^\alpha$ (ours)}



\end{axis}
\end{tikzpicture}

\caption{%Comparison of the developed method on CIFAR-10 versus two baselines: Confidence based on difference of confidence scores and OracleReject. k is the number of classes the expert can predict
}
\label{fig:samplecmplx_auc}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
       title={},
    xlabel={Training data size (as \% of original set)},
    ylabel={mean AU-PR},
    xmin=0, xmax=100,
    ymin=0.61, ymax=0.75,
    xtick={0,5,10,25,50,75,100},
  ytick={0.61,0.62,0.63,0.64,0.65,0.66,0.67,0.68,0.69,0.7,0.71,0.72,0.73,0.74},
    legend pos=north west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 \addplot+[
  black, mark options={black, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    5,  0.624,       0.003
    10,  0.613,       0.005
    25,  0.632,       0.002
    50,  0.661,       0.003
    75,  0.664,       0.004
    100,  0.6612,       0.001
};
\addlegendentry{ModelConfidence}

 \addplot+[
  blue, mark options={blue, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    5,  0.639,       0.002
    10,  0.647,       0.002
    25,  0.680,       0.002
    50,  0.704,       0.003
    75,  0.711,       0.001
    100,  0.701,       0.001
};
\addlegendentry{Confidence}


 \addplot+[
  red, mark options={red, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    5,  0.637,       0.002
    10,  0.669,       0.002
    25,  0.689,       0.002
    50,  0.722,       0.003
    75,  0.733,       0.001
    100,  0.736,       0.001
};
\addlegendentry{$L_{CE}^\alpha$ (ours)}



   \legend{};
\end{axis}
\end{tikzpicture}

\caption{%Comparison of the developed method versus the baselines comparing the accuracy on the non-deferred examples versus the coverage for every $k$. We can see that trained with $L_{CE}^1$, for each expert $L_{CE}$ outperforms the baselines in terms of coverage and classifier accuracy.
}
\label{fig:samplecmplx_pr}
\end{subfigure}
\caption{Left figure shows the average of the maximum achievable AU-ROC for the 5 tasks (average over the tasks) when the changing the size of the training data (as a \% of the original set) and right figure shows the same for AU-PR }
\label{fig:samplecmplx_chexpert}
\end{figure}

\textbf{Results.} In Figure \ref{fig:samplecmplx_chexpert} we plot the average of the maximum achievable AU-ROC \ref{fig:samplecmplx_auc} and AU-PR \ref{fig:samplecmplx_pr} across the 5 tasks for the different methods as we vary the the training set size. We observe that our method consistently outperforms the baselines and continues to take advantage of further data as the baselines performance starts to saturate. If we look at the AU-ROC and AU-PR of the expert on deferred examples, we observe negligible differences as the training set size increases for each method, however if we look at classifier performance on the non-deferred examples, we start to observe a significant difference in AU-ROC and AU-PR for our method while the baselines lag behind. In Figure \ref{fig:plots_classauc_ap_toyexpert} we plot the classifier AU-ROC on non-deferred examples versus the coverage for each of the 5 tasks, we can see for example on Cardiomegaly, our method at full training data obtains an AU-ROC that is at least 0.2 points greater than that of ModelConfidence at coverage levels less than 50\%. One expects  ModelConfidence to achieve the best performance when looking at non-deferred examples, and this in fact is true when we look at accuracy, however for AU-ROC, what happens is that the ModelConfidence baseline never defers on negative predicted examples due to the class imbalance which makes the model very confident in it's negative predictions. Thus, any positive labeled example that the model mistakenly labels as negative with high confidence will cause the AU-ROC to be reduced at low coverage levels. This also allows us to see that our method, and to an extent the Confidence baseline, make very different deferral decisions that factor in the expert.







\begin{figure}[h]
\centering
\begin{subfigure}{.9\textwidth}
\centering

      \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/auc_vs_cov_toyexpert7-1_classifier.pdf}
      \caption{classifier AU-ROC on non-deferred examples vs coverage for expert $q=0.7,p=1$ with 100\% of training data.}
      \label{fig:classauc_vs_cov_toy}
\end{subfigure}

\begin{subfigure}{.9\textwidth}
\centering
  \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/auc_vs_cov_toyexpert7-1_trainsize-0.1_classifier.pdf}
\caption{classifier AU-ROC on non-deferred examples vs coverage for expert $q=0.7,p=1$ with 10\% of training data.}
      \label{fig:classauc_vs_cov_toy_10}
\end{subfigure}

\caption{Plot of classifier AU-ROC on non-deferred examples versus coverage for (a) for systems learned with 100\% of training data  (b) and learned with 10\% of training data. Noise at low coverage is due to reduced data size.}
\label{fig:plots_classauc_ap_toyexpert}
\end{figure}





\subsubsection{Impact of Input Noise}
In our previous experimental setup, the input domain of the classifier $\mathcal{X}$, the chest X-ray, is assumed to be sufficient to perfectly predict the label $Y$ as our golden standard is the prediction of expert radiologists from just looking at the X-ray. Therefore, given enough training data and a sufficiently rich model class, a learned classifier from $\mathcal{X}$ will be able to perfectly predict the target and won't need to defer to any expert to achieve better performance. In this set of experiments, we perform two studies: the first we hide the left part of the chest X-ray on both training and testing examples to obtain a new input domain $\tilde{\mathcal{X}}$. This now limits the power of any learned classifier even in the infinite data regime as the left part of the X-ray may hide crucial parts of the input. 
Figure \ref{fig:noisy_xray} shows this noise applied to a patient's X-ray, the size of the rectangular region was chosen to cover one side of the chest area, we later experiment with varying the scale of the noise.
In the second experiment, we train with the original chest X-rays but evaluate with noisy X-rays with noise in the form of erasing a randomly placed rectangular region of the X-ray. This second experiment is meant to the illustrate the robustness of the different methods to input noise. 

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[scale=0.7,trim={10.0cm 1.0cm 10.0cm 1.0cm}]{figures/xray_original.pdf}
\caption{Original X-ray
}
\label{fig:kvssystem}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[scale=0.7,trim={10.0cm 1.0cm 10.0cm 1.0cm}]{figures/xray_noisy.pdf}

\caption{X-ray with hidden left part
}
\label{fig:covvsacc}
\end{subfigure}
\caption{Left figure (a) shows the chest X-ray of a patient with Cardiomegaly, the right figure (b) shows that same X-ray but now with the left part hidden which is used as input to the models.  }
\label{fig:noisy_xray}
\end{figure}


\textbf{Experimental details.} The noise in the second set of experiments consists of a 2:1 (height:width) randomly located rectangular region of scale (area) that we vary from $0.1$ to $0.66$. The expert is the synthetic expert model with $q=0.7$ and $p=1$.


\textbf{Results.} In Figure \ref{fig:plots_auc_ap_toyexpert_left} we plot the AU-ROC and AU-PR of the different methods as we vary coverage when training and testing while hiding the left section of the X-rays. We can first observe that the maximum achievable performance for the different methods is significantly reduced, however the gap between the different methods is still observed. In Figure \ref{fig:noise_chexpert} we plot the 
average maximum AU-ROC and AU-PR across the 5 tasks as we vary the area of the rectangular region. While the performance of all the methods degrade with the scale of the noise, the gap between the methods remains constant in terms of AU-PR but diminishes in terms of AU-ROC as the performance of the baselines remains steady.





\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={Noise scale},
    ylabel={mean AU-ROC},
    xmin=-0.1, xmax=0.7,
    ymin=0.84, ymax=0.93,
    xtick={0,0.1,0.2,0.33,0.5,0.66},
  ytick={0.85,0.87,0.88,0.89,0.9,0.91,0.92,0.93,0.95},
    legend pos=south west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 \addplot+[
  black, mark options={black, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.879,       0.002
    0.1, 0.878, 0.002
    0.2, 0.873, 0.002
    0.33, 0.870, 0.002
    0.5, 0.868, 0.002
    0.66, 0.868, 0.002

};
\addlegendentry{ModelConfidence}

 \addplot+[
  blue, mark options={blue, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.896,       0.002
    0.1, 0.891, 0.002
    0.2, 0.884, 0.002
    0.33, 0.877, 0.002
    0.5, 0.871, 0.002
    0.66, 0.871, 0.002
};
\addlegendentry{Confidence}


 \addplot+[
  red, mark options={red, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.922,       0.002
    0.1, 0.914, 0.002
    0.2, 0.903, 0.002
    0.33, 0.893, 0.002
    0.5, 0.881, 0.002
    0.66, 0.875, 0.002

};
\addlegendentry{$L_{CE}^\alpha$ (ours)}



\end{axis}
\end{tikzpicture}

\caption{%Comparison of the developed method on CIFAR-10 versus two baselines: Confidence based on difference of confidence scores and OracleReject. k is the number of classes the expert can predict
}
\label{fig:noise_auc}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
       title={},
    xlabel={Noise scale},
    ylabel={mean AU-PR},
    xmin=-0.1, xmax=0.7,
    ymin=0.55, ymax=0.75,
    xtick={0,0.1,0.2,0.33,0.5,0.66},
  ytick={0.55,0.57,0.59,0.61,0.63,0.65,0.67,0.69,0.71,0.73,0.74},
    legend pos=north west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 \addplot+[
  black, mark options={black, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.6612,       0.002
    0.1, 0.648, 0.002
    0.2, 0.612, 0.002
    0.33, 0.595, 0.002
    0.5, 0.572, 0.002
    0.66, 0.560, 0.002
};
\addlegendentry{ModelConfidence}

 \addplot+[
  blue, mark options={blue, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.701,       0.002
    0.1, 0.682, 0.002
    0.2, 0.656, 0.002
    0.33, 0.619, 0.002
    0.5, 0.589, 0.002
    0.66, 0.566, 0.002
};
\addlegendentry{Confidence}


 \addplot+[
  red, mark options={red, scale=0.75},
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.736,       0.002
    0.1, 0.702, 0.002
    0.2, 0.678, 0.002
    0.33, 0.654, 0.002
    0.5, 0.616, 0.002
    0.66, 0.580, 0.002
};
\addlegendentry{$L_{CE}^\alpha$ (ours)}



   \legend{};
\end{axis}
\end{tikzpicture}

\caption{%Comparison of the developed method versus the baselines comparing the accuracy on the non-deferred examples versus the coverage for every $k$. We can see that trained with $L_{CE}^1$, for each expert $L_{CE}$ outperforms the baselines in terms of coverage and classifier accuracy.
}
\label{fig:noise_pr}
\end{subfigure}
\caption{Left figure shows the average of the maximum achievable AU-ROC for the 5 tasks (average over the tasks) when the changing the scale of the noise (size of rectangular region) and right figure shows the same for AU-PR. }
\label{fig:noise_chexpert}
\end{figure}



\begin{figure}[h]
\centering
\begin{subfigure}{.9\textwidth}
\centering

      \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/auc_vs_cov_toyexpert7-1_left.pdf}
      \caption{AU-ROC vs coverage when hiding left part of X-ray.}
      \label{fig:auc_vs_cov_toy_left}
\end{subfigure}

\begin{subfigure}{.9\textwidth}
\centering
  \includegraphics[width=\textwidth,trim={5.0cm 0.0cm 5.0cm 0.0cm}]{figures/ap_vs_cov_toyexpert7-1_left.pdf}
\caption{AU-PR vs coverage when hiding left part of X-ray.}
      \label{fig:ap_vs_cov_toy_left}
\end{subfigure}

\caption{Plots of AU-ROC and AU-PR as we vary coverage when training and testing with chest X-rays that have their left section hidden. The expert model is $q=0.7$ and $p=1$.}
\label{fig:plots_auc_ap_toyexpert_left}
\end{figure}















\section{Radiologist models}

\textbf{2) Radiologist expert.} The hidden test set of 500 patients was labeled by 8 radiologists: the consensus of 5 of them constituted the ground truth label and the annotation of the remaining 3 were used to benchmark radiologist performance. We obtained the ground truth label, the 3 radiologist annotations that were used to benchmark on the test set and the CheXpert automated labels  without the input images. Using  this test data we learn  models of radiologist behavior to use as our expert.
The test data consists of the following tuples $D =\{y_i,e_{1,i},e_{2,i},e_{3,i}\}_{i=1}^{500}$, where $y_i \in \{0,1\}^{14}$ is the CheXpert label, we use the CheXpert labels instead of the concensus to be consistent with the training set, $e_{1,i},e_{2,i},e_{3,i} \in  \{0,1\}^{14}$ are radiologist 1,2 and 3 predictions respectively, the goal is to learn expert models $\hat{e}_1,\hat{e}_2,\hat{e}_3: \{0,1\}^{14} \to \{0,1\}^{14}$ which map a ground truth label to the radiologists predictions. We decompose $\hat{e}_i$ into 14 different components $\hat{e}_i^j:\{0,1\}^{14}  \to \{0,1\}$ (for each of the 14 tasks, $j \in [14]$) and learn each separately.
We evaluate different strategies to learn the expert models: (1) a class conditional noise model (CCN) of the expert based on the task label, (2) a table lookup from the empirical probabilities of $e_i(j)$ ($j$'th component of expert predictions) given the complete label vector $y$, (3) a logistic regression model treating the label vector $y$ as the covariates and $e_i(j)$ as the target (LR) and finally (4) a random forest classifier (RF). \\
\textit{Evaluation of the strategies.} We use 400 patients to train and 100 patients to test the performance of the strategies, and repeat for 50 trials with different random splits to average out the randomness in the models and data. We look in Table \ref{tab:model_rad_behavior} at the area under the ROC curve (AU-ROC) of the expert models at predicting the radiologists decisions for all 3 radiologists and in Table \ref{tab:model_rad_performance} at the average difference between the performance of the expert models in terms of false positive and true positive rates (FPR,TPR) and F1 at predicting the target and the performance of the actual radiologists.

The LR, RF and table lookup method perform similarly at the task of predicting the radiologist decisions  outperforming the naive CCN method, the table lookup method achieves an average AU-ROC of 0.69 over the 5 tasks for radiologist 1. Additionally, all methods are able to match the FPR of the actual experts with an approximate margin of $\pm 0.05$ and the TPR by a margin of $\pm 0.1$ on average across the 3 radiologists. We use the table lookup to construct our expert model for it's simplicity. 



\begin{table}[h]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
         &\textbf{Atelectasis} &  \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Edema} & \textbf{Pleural Effusion}  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 1}} \\ \midrule      
        CCN  & 0.629, (0.585, 0.663)& 0.634, (0.601, 0.664)& 0.568, (0.528, 0.603)& 0.645, (0.606, 0.681)& 0.781, (0.748, 0.806) \\
         \hline
         table lookup & 0.654, (0.613, 0.7)& 0.667, (0.643, 0.701)& 0.625, (0.596, 0.662)& 0.715, (0.695, 0.732)& 0.806, (0.775, 0.841) \\ \hline 
         
      LR &0.646, (0.606, 0.692)& 0.638, (0.606, 0.675)& 0.624, (0.569, 0.669)& 0.719, (0.674, 0.757)& 0.791, (0.761, 0.819) \\ \hline
      
        RF & 0.638, (0.598, 0.67)& 0.657, (0.627, 0.677)& 0.637, (0.593, 0.679)& 0.720, (0.688, 0.753)& 0.806, (0.781, 0.831) \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 2}} \\ \midrule      
        CCN  & 0.672, (0.642, 0.708)& 0.622, (0.592, 0.643)& 0.540, (0.489, 0.574)& 0.633, (0.601, 0.658)& 0.656, (0.631, 0.688) \\
         \hline
         table lookup & 0.697, (0.673, 0.726)& 0.680, (0.643, 0.709)& 0.609, (0.571, 0.65)& 0.668, (0.634, 0.7)& 0.726, (0.691, 0.752) \\ \hline 
         
      LR &0.688, (0.65, 0.713)& 0.669, (0.645, 0.694)& 0.597, (0.532, 0.655)& 0.652, (0.613, 0.691)& 0.710, (0.678, 0.748) \\ \hline
      
        RF &0.702, (0.673, 0.73)& 0.684, (0.643, 0.703)& 0.617, (0.573, 0.66)& 0.672, (0.643, 0.698)& 0.724, (0.687, 0.754) \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 3}} \\ \midrule      
        CCN  & 0.681, (0.631, 0.711)& 0.636, (0.594, 0.671)& 0.571, (0.508, 0.62)& 0.662, (0.631, 0.69)& 0.726, (0.708, 0.735) \\
         \hline
         table lookup & 0.682, (0.636, 0.711)& 0.658, (0.603, 0.707)& 0.594, (0.539, 0.645)& 0.754, (0.722, 0.775)& 0.792, (0.768, 0.822) \\ \hline 
         
      LR &0.700, (0.662, 0.729)& 0.657, (0.614, 0.699)& 0.618, (0.528, 0.689)& 0.758, (0.73, 0.781)& 0.785, (0.76, 0.807) \\ \hline
      
        RF & 0.686, (0.657, 0.714)& 0.679, (0.653, 0.702)& 0.606, (0.539, 0.672)& 0.774, (0.758, 0.789)& 0.795, (0.768, 0.816)
     \\  \bottomrule
    \end{tabular}}
    
    \caption{Average AU-ROC and (25,75) quantiles AU-ROC over the trials of the models at predicting the radiologists predictions for each of the three.}
    \label{tab:model_rad_behavior}
\end{table}








\begin{table}[h]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
         &\textbf{Atelectasis} &  \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Edema} & \textbf{Pleural Effusion}  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 1}} \\ \midrule      
        CCN  & (0.029,0.109), 0.100 & (0.040,0.138), 0.120  & (0.035,0.232), 0.104  & (0.053,0.068), 0.056  & (0.032,0.105), 0.085 \\
         \hline
         table lookup & (0.030,0.124), 0.105 & (0.035,0.113), 0.104  & (0.028,0.252), 0.108  & (0.047,0.073), 0.052  & (0.027,0.110), 0.079 \\ \hline 
         
      LR &(0.031,0.111), 0.097 & (0.034,0.156), 0.122  & (0.035,0.268), 0.135  & (0.043,0.088), 0.056  & (0.022,0.122), 0.086  \\ \hline
      
        RF & (0.034,0.127), 0.120 & (0.032,0.150), 0.118  & (0.034,0.249), 0.115  & (0.043,0.075), 0.048  & (0.022,0.112), 0.079  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 2}} \\ \midrule      
        CCN  & (0.062,0.076), 0.062 & (0.046,0.106), 0.082  & (0.027,0.286), 0.164  & (0.054,0.105), 0.080  & (0.048,0.096), 0.069   \\
         \hline
         table lookup & (0.056,0.059), 0.050 & (0.051,0.106), 0.085  & (0.030,0.222), 0.135  & (0.051,0.095), 0.066  & (0.052,0.093), 0.077  \\ \hline 
         
      LR &(0.050,0.071), 0.044 & (0.056,0.102), 0.083  & (0.033,0.232), 0.147  & (0.051,0.108), 0.082  & (0.054,0.094), 0.070 \\ \hline
      
        RF &(0.060,0.081), 0.058 & (0.045,0.110), 0.070  & (0.027,0.240), 0.156  & (0.047,0.092), 0.062  & (0.044,0.093), 0.069  \\
        \midrule \multicolumn{6}{c}{\textbf{Radiologist 3}} \\ \midrule      
                CCN  &(0.037,0.112), 0.079 & (0.035,0.165), 0.130  & (0.021,0.262), 0.214  & (0.069,0.054), 0.046  & (0.042,0.070), 0.066 \\
         \hline
         table lookup & (0.049,0.101), 0.080 & (0.033,0.131), 0.117  & (0.020,0.252), 0.204  & (0.056,0.063), 0.050  & (0.036,0.085), 0.059 \\ \hline 
         
      LR &(0.044,0.096), 0.079 & (0.038,0.165), 0.130  & (0.023,0.247), 0.194  & (0.062,0.060), 0.046  & (0.038,0.092), 0.064  \\ \hline
      
        RF &(0.044,0.105), 0.077 & (0.030,0.154), 0.117  & (0.040,0.240), 0.226  & (0.054,0.054), 0.039  & (0.033,0.083), 0.052 
      \\  \bottomrule
    \end{tabular}}
    
    \caption{Average absolute difference between the (FPR,TPR) of the expert model at predicting the target and that of the actual radiologists along with the absolute difference of F1 score. }
    \label{tab:model_rad_performance}
\end{table}






==> figures.tex <==
\renewcommand{\familydefault}{\sfdefault}
\clearpage

\begin{figure}
\centering
\centering
\resizebox{3.2in}{!}{%
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={k (classes expert can predict)},
    ylabel={Accuracy},
    xmin=0, xmax=10,
    ymin=88, ymax=100,
    xtick={0,1,2,3,4,5,6,7,8,9,10},
  ytick={88,89,90,91,92,93,94,95,96,97,98,99,100},
    legend pos=north west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (0,90.47)(1,89.54)(2,89.51)(3,89.48)(4,90.75)(5,90.64)(6,93.25)(7,95.28)(8,96.52)(9,98.16)(10,100)
    };
    \addlegendentry{LearnedOracle}

\addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (0,90.47)
    };
    \addlegendentry{Confidence }
    
    \addplot[
    color=red,
    mark=*,
    ]
    coordinates {
    (0,90.47)
    };
    \addlegendentry{$L_{CE}^{.5}$ (ours)}
    
        \addplot[
    color=black,
    mark=*,
    ]
    coordinates {
    (0,90.47)
    };
    \addlegendentry{$L_{CE}^{1}$ (ours)}
    
        \addplot[
    color=violet,
    mark=+,
    ]
    coordinates {
    (0,90.47)(1,90.47)(2,90.47)(3,90.47)(4,90.47)(5,90.47)(6,90.47)(7,90.47)(8,94.48)(9,95.09)(10,100)
    };
    \addlegendentry{MixOfExp }

\end{axis}
\end{tikzpicture}
}%


\end{figure}


\clearpage



\begin{figure}
\centering
\centering
\resizebox{3.2in}{!}{%
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={k (classes expert can predict)},
    ylabel={Accuracy},
    xmin=0, xmax=10,
    ymin=88, ymax=100,
    xtick={0,1,2,3,4,5,6,7,8,9,10},
  ytick={88,89,90,91,92,93,94,95,96,97,98,99,100},
    legend pos=north west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (0,90.47)(1,89.54)(2,89.51)(3,89.48)(4,90.75)(5,90.64)(6,93.25)(7,95.28)(8,96.52)(9,98.16)(10,100)
    };
    \addlegendentry{LearnedOracle}

\addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (0,90.47)(1,90.47)(2,90.56)(3,90.71)(4,91.41)(5,92.52)(6,94.15)(7,95.5)(8,97.35)(9,98.05)(10,100)
    };
    \addlegendentry{Confidence }
    
    \addplot[
    color=red,
    mark=*,
    ]
    coordinates {
    (0,90.47)
    };
    \addlegendentry{$L_{CE}^{.5}$ (ours)}
    
        \addplot[
    color=black,
    mark=*,
    ]
    coordinates {
    (0,90.47)
    };
    \addlegendentry{$L_{CE}^{1}$ (ours)}
    
        \addplot[
    color=violet,
    mark=+,
    ]
    coordinates {
    (0,90.47)(1,90.47)(2,90.47)(3,90.47)(4,90.47)(5,90.47)(6,90.47)(7,90.47)(8,94.48)(9,95.09)(10,100)
    };
    \addlegendentry{MixOfExp }

\end{axis}
\end{tikzpicture}
}%


\end{figure}

\clearpage



\begin{figure}
\centering
\centering
\resizebox{3.2in}{!}{%
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={k (classes expert can predict)},
    ylabel={Accuracy},
    xmin=0, xmax=10,
    ymin=88, ymax=100,
    xtick={0,1,2,3,4,5,6,7,8,9,10},
  ytick={88,89,90,91,92,93,94,95,96,97,98,99,100},
    legend pos=north west,
legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
]

 
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (0,90.47)(1,89.54)(2,89.51)(3,89.48)(4,90.75)(5,90.64)(6,93.25)(7,95.28)(8,96.52)(9,98.16)(10,100)
    };
    \addlegendentry{LearnedOracle}

\addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (0,90.47)(1,90.47)(2,90.56)(3,90.71)(4,91.41)(5,92.52)(6,94.15)(7,95.5)(8,97.35)(9,98.05)(10,100)
    };
    \addlegendentry{Confidence }
    
    \addplot[
    color=red,
    mark=*,
    ]
    coordinates {
    (0,90.47)(1,90.92)(2,91.01)(3,91.94)(4,92.69)(5,93.66)(6,96.03)(7,97.11)(8,98.25)(9,99)(10,100)
    };
    \addlegendentry{$L_{CE}^{.5}$ (ours)}
    
        \addplot[
    color=black,
    mark=*,
    ]
    coordinates {
    (0,90.47)(1,90.41)(2,91)(3,91.47)(4,92.42)(5,93.4)(6,95.07)(7,96.49)(8,97.3)(9,97.7)(10,100)
    };
    \addlegendentry{$L_{CE}^{1}$ (ours)}
        \addplot[
    color=violet,
    mark=+,
    ]
    coordinates {
    (0,90.47)(1,90.47)(2,90.47)(3,90.47)(4,90.47)(5,90.47)(6,90.47)(7,90.47)(8,94.48)(9,95.09)(10,100)
    };
    \addlegendentry{MixOfExp }

\end{axis}
\end{tikzpicture}
}%


\end{figure}
\clearpage



\begin{figure}
\centering

\resizebox{3.2in}{!}{%
\begin{tikzpicture}
\begin{axis}[
    title={},
    xlabel={Coverage (ratio of examples predicted)},
    ylabel={Accuracy on non-deferred examples},
    xmin=0, xmax=100,
    ymin=88, ymax=100,
    xtick={0,10,20,30,40,50,60,70,80,90,100},
    ytick={88,90,91,92,93,94,95,96,97,98,99,100},
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (100,90.47)(90.34,90)(80.33,89.27)(71.71,89.27)(62.43,90.52)(49.65,91.98)(43.12,92.76)(29.03,94.87)(18.34,95.2)(9.2,95.32)(0,100)
    };
    \addlegendentry{LearnedOracle}

\addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (100,90.47)(96.64,90.57)(94.63,90.44)(90.29,90.9)(84.45,91.97)(72.12,92.45)(64.91,93.93)(61.1,94.7)(37.86,94.82)(41.2,96.84)(0,100)
    };
    \addlegendentry{Confidence}
    
    \addplot[
    color=red,
    mark=*,
    ]
    coordinates {
    (100,90.47)(88.78,91.48)(78.66,91.02)(69.02,91.63)(58.47,93.41)(47.72,93.56)(39.05,95.57)(29.15,95.88)(19.41,96.08)(9.53,96.75)(0,100)
    };
    \addlegendentry{$L_{CE}^{.5}$ (ours)}
    
        \addplot[
    color=black,
    mark=*,
    ]
    coordinates {
    (100,90.47)(90.3,91.71)(88,91.7)(91.61,93.1)(76.79,93.92)(71.35,95.42)(61.86,95.28)(49.77,96.49)(46.48,97.3)(47.85,96.54)(0,100)
    };
    \addlegendentry{$L_{CE}^{1}$ (ours)}
         \addplot[
    color=violet,
    mark=+,
    ]
    coordinates {
    (100,90.47)(100,90.47)(100,90.47)(100,90.47)(100,90.47)(100,90.47)(100,90.47)(100,90.47)(46.27,90.47)(40.22,90.47)(0,100)
    };
    \addlegendentry{MixOfExp }   
   \legend{};
\end{axis}
\end{tikzpicture}
}%

\end{figure}


\clearpage

\begin{figure}[h]
\centering
\resizebox{2.8in}{!}{%
\begin{tikzpicture}
\begin{semilogxaxis}[
    title={},
    xlabel={Dataset size (in thousands)},
    ylabel={System accuracy},
    xmin=1, xmax=50,
    ymin=55, ymax=94,
    xtick={1,2,3,5,8,10,20,50},
    ytick={55,58,61,64,67,70,73,76,79,82,85,89,94},
    legend pos=south east,
    log ticks with fixed point,
    ymajorgrids=true,
    yminorticks=false,
    grid style=dashed,
]
 
\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,55.06)(2,62.23)(3,68.02)(5,71.98)(8,79.12)(10,80.46)(20,86.94)(50,92.52)
    };
    \addlegendentry{Confidence}
    

        \addplot[
    color=black,
    mark=*,
    ]
    coordinates {
    (1,62.63)(2,70.12)(3,72.96)(5,75.15)(8,81.1)(10,82.79)(20,88.28)(50,93.4)
    };
    \addlegendentry{$L_{CE}^{1}$ (ours}
\end{semilogxaxis}
\end{tikzpicture}
}%

\end{figure}
\clearpage

